The Leading Behaviour of The Ground-State Energy of Heavy Ions According to Brown and Ravenhall

In this article we prove the absence of relativistic effects in leading order for the ground-state energy according to Brown-Ravenhall operator. We obtain this asymptotic result for negative ions and for systems with the number of electrons proportional to the nuclear charge. In the case of neutral atoms the analogous result was obtained earlier by Cassanas and Siedentop [4].

==> 0258076.tex <==
%auto-ignore
